LiteBIRD Science Goals and Forecasts. A Case Study of the Origin of Primordial Gravitational Waves using Large-Scale CMB Polarization

We study the possibility of using the $LiteBIRD$ satellite $B$-mode survey to constrain models of inflation producing specific features in CMB angular power spectra. We explore a particular model example, i.e. spectator axion-SU(2) gauge field inflation. This model can source parity-violating gravitational waves from the amplification of gauge field fluctuations driven by a pseudoscalar "axionlike" field, rolling for a few e-folds during inflation. The sourced gravitational waves can exceed the vacuum contribution at reionization bump scales by about an order of magnitude and can be comparable to the vacuum contribution at recombination bump scales. We argue that a satellite mission with full sky coverage and access to the reionization bump scales is necessary to understand the origin of the primordial gravitational wave signal and distinguish among two production mechanisms: quantum vacuum fluctuations of spacetime and matter sources during inflation. We present the expected constraints on model parameters from $LiteBIRD$ satellite simulations, which complement and expand previous studies in the literature. We find that $LiteBIRD$ will be able to exclude with high significance standard single-field slow-roll models, such as the Starobinsky model, if the true model is the axion-SU(2) model with a feature at CMB scales. We further investigate the possibility of using the parity-violating signature of the model, such as the $TB$ and $EB$ angular power spectra, to disentangle it from the standard single-field slow-roll scenario. We find that most of the discriminating power of $LiteBIRD$ will reside in $BB$ angular power spectra rather than in $TB$ and $EB$ correlations.

==> authors_affiliations_LB_2021.36_general_jcap-1_old.tex <==
\author[1,2,3]{P.\,Campeti,}
\author[1,4]{E.\,Komatsu,}
\author[5,6,7]{C.\,Baccigalupi,}
\author[8,3,9]{M.\,Ballardini,}
\author[10,11,12]{N.\,Bartolo,}
\author[13,14]{A.\,Carones,}
\author[15]{J.\,Errard,}
\author[9,16]{F.\,Finelli,}
\author[17]{R.\,Flauger,}
\author[18]{S.\,Galli,}
\author[13]{G.\,Galloni,}
\author[19]{S.\,Giardiello,}
\author[20,21,22,4,23]{M.\,Hazumi,}
\author[24]{S.\,Henrot-Versillé,}
\author[25]{L.\,T.\,Hergt,}
\author[21]{K.\,Kohri,}
\author[4]{C.\,Leloup,}
\author[26]{J.\,Lesgourgues,}
\author[27]{J.\,Macias-Perez,}
\author[28]{E.\,Martínez-González,}
\author[10,11,12,29]{S.\,Matarrese,}
\author[4]{T.\,Matsumura,}
\author[30]{L.\,Montier,}
\author[4]{T.\,Namikawa,}
\author[9,16]{D.\,Paoletti,}
\author[31,32]{D.\,Poletti,}
\author[28,33]{M.\,Remazeilles,}
\author[34]{M.\,Shiraishi,}
\author[24]{B.\,van\,Tent,}
\author[24]{M.\,Tristram,}
\author[5]{L.\,Vacher,}
\author[13,14]{N.\,Vittorio,}
\author[24]{G.\,Weymann-Despres,}
\author[13]{A.\,Anand,}
\author[30]{J.\,Aumont,}
\author[35]{R.\,Aurlien,}
\author[30]{A.\,J.\,Banday,}
\author[28]{R.\,B.\,Barreiro,}
\author[35]{A.\,Basyrov,}
\author[36,37]{M.\,Bersanelli,}
\author[38,39]{D.\,Blinov,}
\author[8,3]{M.\,Bortolami,}
\author[8]{T.\,Brinckmann,}
\author[19]{E.\,Calabrese,}
\author[5]{F.\,Carralot,}
\author[28]{F.\,J.\,Casas,}
\author[40]{L.\,Clermont,}
\author[41,42]{F.\,Columbro,}
\author[31]{G.\,Conenna,}
\author[41,42]{A.\,Coppolecchia,}
\author[9]{F.\,Cuttaia,}
\author[41,42]{G.\,D'Alessandro,}
\author[41,42]{P.\,de\,Bernardis,}
\author[41,42]{M.\,De\,Petris,}
\author[32]{S.\,Della\,Torre,}
\author[43]{E.\,Di\,Giorgi,}
\author[28,44]{P.\,Diego-Palazuelos,}
\author[35]{H.\,K.\,Eriksen,}
\author[36,37]{C.\,Franceschet,}
\author[35]{U.\,Fuskeland,}
\author[35]{M.\,Galloway,}
\author[40]{M.\,Georges,}
\author[3]{M.\,Gerbino,}
\author[31,32]{M.\,Gervasi,}
\author[20]{T.\,Ghigna,}
\author[28]{C.\,Gimeno-Amo,}
\author[35]{E.\,Gjerløw,}
\author[9,16]{A.\,Gruppuso,}
\author[56]{J.\,Gudmundsson}
\author[5,6,7]{N.\,Krachmalnicoff,}
\author[41,42]{L.\,Lamagna,}
\author[3]{M.\,Lattanzi,}
\author[8]{M.\,Lembo,}
\author[13]{A.\,I.\,Lonappan,}
\author[41,42]{S.\,Masi,}
\author[43]{M.\,Massa,}
\author[41]{S.\,Micheli,}
\author[43]{A.\,Moggi,}
\author[1]{M.\,Monelli,}
\author[9]{G.\,Morgante,}
\author[30]{B.\,Mot,}
\author[45,30]{L.\,Mousset,}
\author[22]{R.\,Nagata,}
\author[8,3]{P.\,Natoli,}
\author[41]{A.\,Novelli,}
\author[4]{I.\,Obata,}
\author[8,3,46]{L.\,Pagano,}
\author[41,42]{A.\,Paiella,}
\author[38,39]{V.\,Pavlidou,}
\author[41,42]{F.\,Piacentini,}
\author[43]{M.\,Pinchera,}
\author[41]{G.\,Pisano,}
\author[47,48,49]{G.\,Puglisi,}
\author[8]{N.\,Raffuzzi,}
\author[50,45]{A.\,Ritacco,}
\author[15]{A.\,Rizzieri,}
\author[28,44]{M.\,Ruiz-Granda,}
\author[51]{G.\,Savini,}
\author[25]{D.\,Scott,}
\author[43]{G.\,Signorelli,}
\author[52,4]{S.\,L.\,Stever,}
\author[35]{N.\,Stutzer,}
\author[25]{R.\,M.\,Sullivan,}
\author[43,53]{A.\,Tartari,}
\author[38,39]{K.\,Tassis,}
\author[9]{L.\,Terenzi,}
\author[54,55]{K.\,L.\,Thompson,}
\author[28]{P.\,Vielva,}
\author[35]{I.\,K.\,Wehus,}
\author[20]{and Y.\,Zhou}
\author[ ]{\\LiteBIRD Collaboration.}
\affiliation[1]{Max Planck Institute for Astrophysics, Karl-Schwarzschild-Str. 1, D-85748 Garching, Germany}
\affiliation[2]{Excellence Cluster ORIGINS, Boltzmannstr. 2, 85748 Garching, Germany}
\affiliation[3]{INFN Sezione di Ferrara, Via Saragat 1, 44122 Ferrara, Italy}
\affiliation[4]{Kavli Institute for the Physics and Mathematics of the Universe (Kavli IPMU, WPI), UTIAS, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan}
\affiliation[5]{International School for Advanced Studies (SISSA), Via Bonomea 265, 34136, Trieste, Italy}
\affiliation[6]{INFN Sezione di Trieste, via Valerio 2, 34127 Trieste, Italy}
\affiliation[7]{IFPU, Via Beirut, 2, 34151 Grignano, Trieste, Italy}
\affiliation[8]{Dipartimento di Fisica e Scienze della Terra, Università di Ferrara, Via Saragat 1, 44122 Ferrara, Italy}
\affiliation[9]{INAF - OAS Bologna, via Piero Gobetti, 93/3, 40129 Bologna, Italy}
\affiliation[10]{Dipartimento di Fisica e Astronomia “G. Galilei”, Universita` degli Studi di Padova, via Marzolo 8, I-35131 Padova, Italy}
\affiliation[11]{INFN Sezione di Padova, via Marzolo 8, I-35131, Padova, Italy}
\affiliation[12]{INAF, Osservatorio Astronomico di Padova, Vicolo dell’Osservatorio 5, I-35122, Padova, Italy}
\affiliation[13]{Dipartimento di Fisica, Università di Roma Tor Vergata, Via della Ricerca Scientifica, 1, 00133, Roma, Italy}
\affiliation[14]{INFN Sezione di Roma2, Università di Roma Tor Vergata, via della Ricerca Scientifica, 1, 00133 Roma, Italy}
\affiliation[15]{Université de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\affiliation[16]{INFN Sezione di Bologna, Viale C. Berti Pichat, 6/2 – 40127 Bologna Italy}
\affiliation[17]{University of California, San Diego, Department of Physics, San Diego, CA 92093-0424, USA}
\affiliation[18]{Institut d'Astrophysique de Paris, CNRS/Sorbonne Université, Paris France}
\affiliation[19]{School of Physics and Astronomy, Cardiff University, Cardiff CF24 3AA, UK}
\affiliation[20]{International Center for Quantum-field Measurement Systems for Studies of the Universe and Particles (QUP), High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}
\affiliation[21]{Institute of Particle and Nuclear Studies (IPNS), High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}
\affiliation[22]{Japan Aerospace Exploration Agency (JAXA), Institute of Space and Astronautical Science (ISAS), Sagamihara, Kanagawa 252-5210, Japan}
\affiliation[23]{The Graduate University for Advanced Studies (SOKENDAI), Miura District, Kanagawa 240-0115, Hayama, Japan}
\affiliation[24]{Université Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affiliation[25]{Department of Physics and Astronomy, University of British Columbia, 6224 Agricultural Road, Vancouver BC, V6T1Z1, Canada}
\affiliation[26]{Institute for Theoretical Particle Physics and Cosmology (TTK), RWTH Aachen, 52056 Aachen, Germany}
\affiliation[27]{Université Grenoble Alpes, CNRS, LPSC-IN2P3, 53, avenue des Martyrs, 38000 Grenoble, France}
\affiliation[28]{Instituto de Fisica de Cantabria (IFCA, CSIC-UC), Avenida los Castros SN, 39005, Santander, Spain}
\affiliation[29]{Gran Sasso Science Institute (GSSI), Viale F. Crispi 7, I-67100, L’Aquila, Italy}
\affiliation[30]{IRAP, Université de Toulouse, CNRS, CNES, UPS, (Toulouse), France}
\affiliation[31]{University of Milano Bicocca, Physics Department, p.zza della Scienza, 3, 20126 Milan Italy}
\affiliation[32]{INFN Sezione Milano Bicocca, Piazza della Scienza, 3, 20126 Milano, Italy}
\affiliation[33]{Jodrell Bank Centre for Astrophysics, Alan Turing Building, Department of Physics and Astronomy, School of Natural Sciences, The University of Manchester, Oxford Road, Manchester M13 9PL, UK}
\affiliation[34]{Suwa University of Science, Chino, Nagano 391-0292, Japan}
\affiliation[35]{Institute of Theoretical Astrophysics, University of Oslo, Blindern, Oslo, Norway}
\affiliation[36]{Dipartimento di Fisica, Universita' degli Studi di Milano, Via Celoria 16 - 20133, Milano, Italy}
\affiliation[37]{INFN Sezione di Milano, Via Celoria 16 - 20133, Milano, Italy}
\affiliation[38]{Institute of Astrophysics, Foundation for Research and Technology-Hellas, Vasilika Vouton, GR-70013 Heraklion, Greece}
\affiliation[39]{Department of Physics and ITCP, University of Crete, GR-70013, Heraklion, Greece}
\affiliation[40]{Centre Spatial de Liège, Université de Liège, Avenue du Pré-Aily, 4031 Angleur, Belgium}
\affiliation[41]{Dipartimento di Fisica, Università La Sapienza, P. le A. Moro 2, Roma, Italy}
\affiliation[42]{INFN Sezione di Roma, P.le A. Moro 2, 00185 Roma, Italy}
\affiliation[43]{INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127 Pisa, Italy}
\affiliation[44]{Dpto. de Física Moderna, Universidad de Cantabria, Avda. los Castros s/n, E-39005 Santander, Spain}
\affiliation[45]{Laboratoire de Physique de l’École Normale Supérieure, ENS, Université PSL, CNRS, Sorbonne Université, Université de Paris, 75005 Paris, France}
\affiliation[46]{Université Paris-Saclay, CNRS, Institut d’Astrophysique Spatiale, 91405, Orsay, France}
\affiliation[47]{Dipartimento di Fisica e Astronomia, Universitá degli Studi di Catania, Via S. Sofia,64, 95123, Catania, Italy}
\affiliation[48]{INAF, Osservatorio Astrofisico di Catania, via S.Sofia 78, I-95123 Catania, Italy}
\affiliation[49]{INFN, Sezione di Catania, via S.Sofia 64, I-95123, Catania, Italy}
\affiliation[50]{INAF, Osservatorio Astronomico di Cagliari, Via della Scienza 5, 09047 Selargius, Italy}
\affiliation[51]{Physics and Astronomy Dept., University College London (UCL), UK}
\affiliation[52]{Okayama University, Department of Physics, Okayama 700-8530, Japan}
\affiliation[53]{Dipartimento di Fisica, Università di Pisa, Largo B. Pontecorvo 3, 56127 Pisa, Italy}
\affiliation[54]{SLAC National Accelerator Laboratory, Kavli Institute for Particle Astrophysics and Cosmology (KIPAC),  Menlo Park, CA 94025, USA}
\affiliation[55]{Stanford University, Department of Physics,  CA 94305-4060, USA}
\affiliation[56]{The Oskar Klein Centre, Department of Physics, Stockholm University, AlbaNova, SE-10691 Stockholm, Sweden}
